Surfacing Estimation Uncertainty in the Decay Parameters of Hawkes Processes with Exponential Kernels

As a tool for capturing irregular temporal dependencies (rather than resorting to binning temporal observations to construct time series), Hawkes processes with exponential decay have seen widespread adoption across many application domains, such as predicting the occurrence time of the next earthquake or stock market spike. However, practical applications of Hawkes processes face a noteworthy challenge: There is substantial and often unquantified variance in decay parameter estimations, especially in the case of a small number of observations or when the dynamics behind the observed data suddenly change. We empirically study the cause of these practical challenges and we develop an approach to surface and thereby mitigate them. In particular, our inspections of the Hawkes process likelihood function uncover the properties of the uncertainty when fitting the decay parameter. We thus propose to explicitly capture this uncertainty within a Bayesian framework. With a series of experiments with synthetic and real-world data from domains such as "classical" earthquake modeling or the manifestation of collective emotions on Twitter, we demonstrate that our proposed approach helps to quantify uncertainty and thereby to understand and fit Hawkes processes in practice.

==> sections/results.tex <==
\section{Results}\label{sec:empirical_analysis}

\begin{figure*}[!t]
	\begin{center}
		\subfloat[Far View]{
			\includegraphics[width=0.31\textwidth]{results/loglik/updated_loglik_plot_Far_mean_ci}
			\label{fig:loglik_far}
		}
		\subfloat[Close View]{
			\includegraphics[width=0.31\textwidth]{results/loglik/updated_loglik_plot_Broad_mean_ci}
			\label{fig:loglik_broad}
		}
		\subfloat[Closest View]{
			\includegraphics[width=0.31\textwidth]{results/loglik/updated_loglik_plot_Close_mean}
			\label{fig:loglik_close}
		}
		\caption{\label{fig:loglik}
			%\small
			\textbf{Convex-Like Noisy Log-Likelihood of Hawkes Processes as a Function of the Decay Parameter Beta ($\beta$).} 
			We simulate realizations from a two-dimensional Hawkes process with a given beta value for both dimensions ($\beta=1.2$), and we evaluate its log-likelihood for a large (cf. Fig.~\ref{fig:loglik_far}), medium (cf. Fig.~\ref{fig:loglik_broad}) and small (cf. Fig.~\ref{fig:loglik_close}) range of decay parameter values around the given one. Error bars throughout this paper indicate boostrapped $95\%$ confidence intervals, which may be too small to be visible\textsuperscript{a}. While the log-likelihood appears convex on a high-level, zooming in around the given value reveals a wide and noisy basin, which explains difficulties in optimizing the log-likelihood for the decay parameter. This finding is robust across Hawkes process parameter configurations which satisfy the stationarity constraint.
		}
	\end{center}
	\small\textsuperscript{a} Single exception: We omit the error bars in Fig.~\ref{fig:loglik_close} for visualization purposes (as the error bars would otherwise overlap and render the Figure unintelligible).
\end{figure*}

\begin{figure*}[!t]
	\begin{center}
		\subfloat[Log-Likelihood (Full)]{
			\includegraphics[width=0.23\textwidth]{results/cvx_others/Log Likelihood}
			\label{fig:cvx_others_loglik_full}
		}
		\subfloat[K-S Distance (Full)]{
			\includegraphics[width=0.23\textwidth]{results/cvx_others/K-S Distance}
			\label{fig:cvx_others_ks_full}
		}
		\subfloat[RMSE (Full)]{
			\includegraphics[width=0.23\textwidth]{results/cvx_others/RMSE}
			\label{fig:cvx_others_rmse_full}
		}
		\subfloat[Time (Full)]{
			\includegraphics[width=0.23\textwidth]{results/cvx_others/Time (s)}
			\label{fig:cvx_others_time_full}
		}\\
		\subfloat[Log-Likelihood (Excerpt)]{
			\includegraphics[width=0.23\textwidth]{results/cvx_others/Log Likelihood_noWrong+}
			\label{fig:cvx_others_loglik_excerpt}
		}
		\subfloat[K-S Distance (Excerpt)]{
			\includegraphics[width=0.23\textwidth]{results/cvx_others/K-S Distance_noWrong+}
			\label{fig:cvx_others_ks_excerpt}
		}
		\subfloat[RMSE (Excerpt)]{
			\includegraphics[width=0.23\textwidth]{results/cvx_others/RMSE_noWrong}
			\label{fig:cvx_others_rmse_excerpt}
		}
		\subfloat[Time (Excerpt)]{
			\includegraphics[width=0.23\textwidth]{results/cvx_others/Time (s)_noFit}
			\label{fig:cvx_others_time_excerpt}
		}
		\caption{\label{fig:cvx_others}
			%\small
			\textbf{All Approaches for Fitting Beta Perform Comparably Well.}
			We simulate $100$ stationary two-dimensional Hawkes processes with random parameter values, and we evaluate the beta estimation approaches ``nonlinear optimization'' (``Fitted Beta'' in the Figures), ``expectation maximization'' (``Exp. Max.''), ``grid search'' (``Grid Beta'') and ``hyperparameter optimization'' (``Hyperopt''). As baselines for those four approaches, we also compute the fit quality with a fixed beta that is correct (``Given Beta''), a wrong beta in the same order of magnitude (``Wrong Beta''), as well as one (``Wrong Beta+'') and two (``Wrong Beta++'') orders of magnitude greater than the correct one. The upper row of Figures contains all approaches and the lower row selected ones for visualization purposes. We measure performance along a series of metrics, namely Hawkes process log-likelihood (``Log Likelihood''; Figs.~\ref{fig:cvx_others_loglik_full},~\ref{fig:cvx_others_loglik_excerpt}), Kolmogorov-Smirnov distances between simulated and real event streams (``K-S Distance''; Figs.~\ref{fig:cvx_others_ks_full},~\ref{fig:cvx_others_ks_excerpt}), root mean squared error of fitted and real decay parameter values (``RMSE''; Figs.~\ref{fig:cvx_others_rmse_full},~\ref{fig:cvx_others_rmse_excerpt}), and run-time of the fitting procedure using commodity hardware (``Time (s)''; Figs.~\ref{fig:cvx_others_time_full},~\ref{fig:cvx_others_time_excerpt}). For all metrics, lower values are better. Except when guessed values for beta are remarkably wrong, all approaches perform comparably well, with nonlinear optimization attaining a slightly better fit at the cost of runtime.
		}
	\end{center}
\end{figure*}

\begin{figure*}[!t]
	\begin{center}
		\subfloat[One Beta]{
			\includegraphics[width=0.45\columnwidth]{results/causal/causality_acc_2dim_1beta}
			\label{fig:causal_1beta}
		}
		\subfloat[Four Betas]{
			\includegraphics[width=0.45\columnwidth]{results/causal/causality_acc_2dim_4beta}
			\label{fig:causal_4beta}
		}
		\caption{\label{fig:causal}
			%\small
			\textbf{Significantly Wrong Beta Estimations Impact Directionality of Influence.}
			Using the same simulation setup and notation as in Fig.~\ref{fig:cvx_others}, we measure and depict the accuracy of inferred influence directionality between Hawkes process dimensions. We define this accuracy as the relative frequency of how often the ranking of the estimated cross-excitation values corresponds to the real one. Higher values are better. We repeat this simulation for two-dimensional processes with one beta only (cf. Fig.~\ref{fig:causal_1beta}) as well as four different betas (cf. Fig.~\ref{fig:causal_4beta}), and we find remarkably wrong betas may lead to errors in the estimation of influence directionality. Again, higher dimensionality and number of betas leads to decreasing performance.
		}
	\end{center}
\end{figure*}

\begin{figure*}[!t]
	\begin{center}
		\includegraphics[width=0.95\columnwidth]{results/real/real_world_duolingo_ratio}
		\caption{\label{fig:duolingo}
			%\small
			\textbf{In the Duolingo App, Users Learning C-level Words Have Longer Learning Bursts Than Those Learning A-level Words.}
			We fit two Hawkes processes to users learning vocabulary on Duolingo: one process and its realization consist of a user learning ``hard'' (i.e. C-level) words, and the other of a user learning ``easy'' (i.e. A-level) words. We control for total activity levels by considering only users with ten learning events per word difficulty. Our results are robust to this choice of event total. We depict the ratio of the decay value of the C-level words to the A-level words, and we hypothesize the former is half as large as the latter. The fitted values show this ratio is even lower (``Fitted Beta Ratio'') in comparison to the ratio of posteriors (``Bayesian Beta Ratio''). Overall, lower decay values for the same number of events imply a more prolonged learning burst, suggesting learning C-level words requires more sustained effort from users.
		}
	\end{center}
\end{figure*}

\begin{figure*}[!t]
	\begin{center}
		\includegraphics[width=0.95\columnwidth]{results/real/real_world_emotions_beta_20-25_8d_subsample}
		\caption{\label{fig:emotions}
			%\small
			\textbf{Tweet Timing Reflects Collective Emotions.}
			We depict the result of fitting an MCMC-based changepoint detection model to users' Tweet timings in the two weeks surrounding the November 2015 Paris attacks (while again controlling for total tweet count per user): The estimated density for the Hawkes process intensity decay assigns more probability mass to higher decay regions before the change (``Beta 1'') in comparison to after (``Beta 2''). These findings are, again, robust to the choice of user activity level. This suggests collective effervescence manifests on Tweet timings as well. \tsa{Denis, please remind me to discuss the following:} One limitation of this changepoint detection approach lies in the estimation of when the change happens, which is about $20\%$ later than what should be.
		}
	\end{center}
\end{figure*}

Results

